Adaptive minimax testing for circular convolution

Given observations from a circular random variable contaminated by an additive measurement error, we consider the problem of minimax optimal goodness-of-fit testing in a non-asymptotic framework. We propose direct and indirect testing procedures using a projection approach. The structure of the optimal tests depends on regularity and ill-posedness parameters of the model, which are unknown in practice. Therefore, adaptive testing strategies that perform optimally over a wide range of regularity and ill-posedness classes simultaneously are investigated. Considering a multiple testing procedure, we obtain adaptive i.e. assumption-free procedures and analyse their performance. Compared with the non-adaptive tests, their radii of testing face a deterioration by a log-factor. We show that for testing of uniformity this loss is unavoidable by providing a lower bound. The results are illustrated considering Sobolev spaces and ordinary or super smooth error densities.

==> packages.tex <==
% 
\usepackage[english]{babel}
\RequirePackage{ucs}
\RequirePackage[utf8x]{inputenc}
%
% zeige labels am rand an.
%\usepackage[notref,notcite]{showkeys} 
%  aendere Anzeige der labels         
%\renewcommand{\showkeyslabelformat}[1]{%
%	\mbox{\dg \normalfont\tiny\ttfamily#1}}
%%
%
\usepackage{lmodern} % font: Latin Modern
\usepackage[right = 2cm, top=2.5cm, bottom=2.5cm,left=2cm]{geometry}
%
%
%
%
%==========================================
\RequirePackage{amsthm,amsmath}
\RequirePackage{amssymb,amstext}
\RequirePackage{amsfonts,stmaryrd}
\RequirePackage{amsbsy} 
\RequirePackage{mathrsfs}
\RequirePackage{bm}
\RequirePackage{bbm}
\RequirePackage{aliascnt,ifthen}
\RequirePackage{graphicx}
\RequirePackage{color,calc}
\RequirePackage{url}
\RequirePackage{verbatim}
\RequirePackage{thmtools}
\RequirePackage{mathtools}
\RequirePackage{relsize}

\usepackage[pdfpagemode=UseOutlines ,plainpages=false,
%hypertexnames=false ,pdfpagelabels=TRUE ,
hyperindex=true,colorlinks=true]{hyperref}
	\makeatletter
	\Hy@breaklinkstrue
	\makeatother


\hypersetup{colorlinks ,linkcolor=gray ,filecolor=darkgreen,  urlcolor=blue ,citecolor=black}

\RequirePackage{paralist}

% BIBLIOGRAPHY
\usepackage{natbib}
\usepackage{hypernat}
\renewcommand{\cite}{\citet}
\bibliographystyle{abbrvnat}

%==========================================
% Packages sandra
%==========================================
\usepackage{enumitem} % advanced enumeration
\usepackage{graphicx} % for including graphics
\usepackage{dsfont} % indicator function \mathds{1}
\usepackage{tikz} % tikz pgf: advanced drawing
\usetikzlibrary{shapes.geometric, arrows.meta, calc, positioning, shapes.multipart}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{ifthen}
\usepackage{supertabular} % tables with pagebreaks
\usepackage{booktabs}  % nicer tables
\usepackage{cases}
\usepackage{xcolor}
%
\usepackage{blindtext}
\usepackage{multirow}

%==========================================
% Packages jan
%==========================================
\usepackage{cleveref}
\crefname{definition}{\color{\colde}Definition}{\color{\colde}Definitions}
\crefname{lemma}{\color{\colre}Lemma}{\color{\colre}Lemmata}
\crefname{proposition}{\color{\colre}Proposition}{\color{\colre}Propositions}
\crefname{requisite}{\color{\colrem}Requisite}{\color{\colrem}Requisites}
\crefname{theorem}{\color{\colre}Theorem}{\color{\colre}Theorems}
\crefname{corollary}{\color{\colre}Corollary}{\color{\colre}Corollaries}
\crefname{remark}{\color{\colrem}Remark}{\color{\colrem}Remarks}
\crefname{assumption}{\color{\colrem}Assumption}{\color{\colrem}Assumptions}
\crefname{illustration}{\color{\colil}Illustration}{\color{\colil}Illustrations}
\crefname{section}{\color{\colre}Section}{\color{\colre}Sections}
\crefname{appendix}{\color{\colre}Appendix}{\color{\colre}Appendices}
\numberwithin{equation}{section} 


